All-in-One: Heterogeneous Interaction Modeling for Cold-Start Rating Prediction

Cold-start rating prediction is a fundamental problem in recommender systems that has been extensively studied. Many methods have been proposed that exploit explicit relations among existing data, such as collaborative filtering, social recommendations and heterogeneous information network, to alleviate the data insufficiency issue for cold-start users and items. However, the explicit relations constructed based on data between different roles may be unreliable and irrelevant, which limits the performance ceiling of the specific recommendation task. Motivated by this, in this paper, we propose a flexible framework dubbed heterogeneous interaction rating network (HIRE). HIRE dose not solely rely on the pre-defined interaction pattern or the manually constructed heterogeneous information network. Instead, we devise a Heterogeneous Interaction Module (HIM) to jointly model the heterogeneous interactions and directly infer the important interactions via the observed data. In the experiments, we evaluate our model under three cold-start settings on three real-world datasets. The experimental results show that HIRE outperforms other baselines by a large margin. Furthermore, we visualize the inferred interactions of HIRE to confirm the contribution of our model.

==> bak.tex <==
%sampling

Since the main idea of Cube Transformer is to utilize information between instances to learn the interaction in the recommendation system, we input a minibatch of users and items to make \CT work. We sample a task matrix with the following requirements: 
1) We should promise for all the users in tasks, they have interaction with sampled items to make sure that recommendation can be made for these users;
2) To get relative complete information, we should sample users who have common item interactions with other users and also those who do not have interaction with these items. 
%todo3) 
To satisfy these requirements, we device a simple one-hop sampling strategy to sample a task given a user and an item.
The one-hop sampling strategy first randomly sample a user $u_1$ and a set of $D$ items that the user $u_1$ has rating before. For each user in dataset, extract those users that has some interactions with items in the item set $\mathcal{I}$.
The details of our sampling strategy is summarized in Algorithm 1.
\begin{algorithm}[h]
	\footnotesize
	\caption{Sampling strategy}
	\label{alg}
	\DontPrintSemicolon
	\SetKwData{Up}{up}  \SetKwInOut{Input}{Input} \SetKwInOut{Output}{Output}
	\Input{User set $U$, Item set $I$, sampling size of users $N$, sampling size of items $D$, user-item interaction matrix $M$}
	\Output{Sampled user set $\mathcal{U}$, Sampled item set $\mathcal{I}$}
	\SetKwFunction{Emit}{Emit}
	\SetKwFunction{Check}{Check}

	Random sample a user $u_1$, append $u_1$ to user set $\mathcal{U}$;\;
        Sample a set of items that user $u_1$ has interaction history with size of $D$, append items to item set $\mathcal{I}$;\;
        
		\For { $u \in U$ } 
		{ 
                initialize $\text{count}[u]$=0;\;
			\For {$v \in \mathcal{I}$}
			{ 
                    \If {$u$ has rating $v$ before}
                     {$count[u]++$;}
			}}
        Sort $\text{count}$ in descending order;\;
        Random sample $D-1$ users from top $2N$ $\text{count}$, append them into set $\mathcal{U}$.\;
	\Return{$\mathcal{U}$, $\mathcal{I}$};\
\end{algorithm}
User set $\mathcal{U}$; Item set $\mathcal{I}$; User and item feature; Explicit ratings.



%preliminary
\subsection{Multi-Head Self-Attention}
\label{subsec:mhsa}
Multi-head self-attention (MHSA) has been widely applied in natural language process \cite{BERT, allyouneed}. Recently, research efforts extend the attention mechanism for tabular data \cite{transformer4tabular, annocolumn, NPT}. Multi-head self-attention allows the model to learn complex interactions between input sequence instances.
Attention function $\text{Att}(Q,K,V)$ maps queries $Q\in \mathbb{R}^{n\times h_k}$ to outputs using key-value pairs, the keys and values are packed together into matrices $K\in \mathbb{R}^{m\times h_k}$ and $V\in \mathbb{R}^{m\times h_v}$.
We compute dot-product attention,
\begin{align}
	\text{Att}(Q,K,V) &= \text{softmax}(QK^T/\sqrt{h})V. \label{eq:attention}
\end{align}
The pairwise dot product $QK^T$ measures the similarity between each pair of query and key vectors. The output is a weighted sum of $V$.
Instead perform a single dot product attention, a series of $k$ independent attention heads are concatenated, which allows the model to jointly attend to knowledge from different subspace. Multi-head attention is computed as follows,

\begin{align}
	\text{MHA}(Q,K,V) &= \text{concat}(O_1,\dots,O_k)W^O, \space \text{where} \label{eq:mhsa} \\
	O_j &= \text{Att}(QW_j^Q,KW_j^K,VW_j^V).
\end{align}
where $W_j^Q,W_j^K,W_j^V ,W^O$ are learnable parameters.
In this paper, we use multi-head self-attention, $\text{MHSA}(H)=\text{MHA}(Q=H,K=H,V=H)$, which set the same value for query $Q$, key $K$ and value $V$.


%and $y_{uv}=-1$ if no rating was given by user $u$ to item $v$ before or their interactions are not observed.


\comment{
\begin{table*}[h]
\small
\centering
\caption{Performance on Three Cold-Start Scenario}
\label{tab:result}
\resizebox{1\textwidth}{!}
{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
                           &                           & \multicolumn{6}{c|}{\UC}                                                                                                                                                          & \multicolumn{6}{c|}{\IC}                                                                                                                                                          & \multicolumn{6}{c|}{\UIC}                                                                                                                                     \\\cline{3-20}
                           &                           & \multicolumn{3}{c|}{TOP5}                                                     & \multicolumn{3}{c|}{TOP10}                                                                        & \multicolumn{3}{c|}{TOP5}                                                     & \multicolumn{3}{c|}{TOP10}                                                                        & \multicolumn{3}{c|}{TOP5}                                                     & \multicolumn{3}{c|}{TOP10}                                                    \\\cline{3-20}
\multirow{-3}{*}{Datasets} & \multirow{-3}{*}{Methods} & \multicolumn{1}{c|}{\PRE} & \multicolumn{1}{c|}{\NDCG} & \multicolumn{1}{c|}{\MAP} & \multicolumn{1}{c|}{\PRE}        & \multicolumn{1}{c|}{\NDCG}       & \multicolumn{1}{c|}{\MAP}        & \multicolumn{1}{c|}{\PRE} & \multicolumn{1}{c|}{\NDCG} & \multicolumn{1}{c|}{\MAP} & \multicolumn{1}{c|}{\PRE}        & \multicolumn{1}{c|}{\NDCG}       & \multicolumn{1}{c|}{\MAP}        & \multicolumn{1}{c|}{\PRE} & \multicolumn{1}{c|}{\NDCG} & \multicolumn{1}{c|}{\MAP} & \multicolumn{1}{c|}{\PRE} & \multicolumn{1}{c|}{\NDCG} & \multicolumn{1}{c|}{\MAP} \\\hline
\multirow{8}{*}\Movielens                  & \NEUMF                     & 0.4864                  & 0.7856                   & 0.3589                  & 0.7171                         & 0.8371                         & 0.5938                         & 0.5039                  & 0.6645                   & 0.3731                  & 0.7864                         & 0.7662                         & 0.6972                         & 0.5049                  & 0.6695                   & 0.3756                  & 0.7875                  & 0.7691                   & 0.7009                  \\
                           & \WIDE                      & 0.6079                  & \cellcolor{LightYellow}0.8585                   & 0.5144                  & 0.7713                         & 0.8849                         & 0.6915                         & 0.4776                  & 0.6314                   & 0.3605                  & 0.7357                         & 0.7105                         & 0.6313                         & 0.4864                  & 0.6405                   & 0.3657                  & 0.7338                  & 0.7157                   & 0.6309                  \\
                           & \DEEPFM                    & 0.6060                   & 0.8562                   & 0.5088                  & 0.7707                         & 0.8848                         & 0.6909                         & 0.4626                  & 0.6166                   & 0.3391                  & 0.7343                         & 0.7020                          & 0.6263                         & 0.4657                  & 0.6200                     & 0.3377                  & 0.7355                  & 0.7059                   & 0.6247                  \\
                           & \AFN                       & 0.5899                  & 0.8479                   & 0.4862                  & 0.7712                         & 0.8808                         & 0.6869                         & 0.4496                  & 0.6003                   & 0.3288                  & 0.7268                         & 0.6888                         & 0.614                          & 0.4745                  & 0.6334                   & 0.3583                  & 0.7161                  & 0.6998                   & 0.6131                  \\
                           & \TANP                      & 0.627                   & 0.8717                   & 0.5333                  & 0.7797                         & 0.8987                         & 0.6994                         & 0.5488                  & 0.8072                   & 0.4257                  & 0.7544                         & 0.8528                         & 0.6492                         & 0.5371                  & 0.8069                   & 0.412                   & 0.7467                  & 0.8516                   & 0.642                   \\
                           & \MELU                      & \cellcolor{LightYellow}0.7104                  & 0.7852                   & 0.6275                  & 0.8868                         & 0.8589                         & 0.8469                         & 0.7119                  & 0.7856                   & 0.628                   & 0.8874                         & 0.8589                         & 0.8473                         & 0.7102                  & 0.7842                   & 0.6267                  & 0.8883                  & 0.8585                   & 0.8479                  \\
                           & \MAMO                      & 0.5428                  & 0.6327                   & 0.4241                  & 0.7661                         & 0.7187                         & 0.6678                         & 0.5371                  & 0.6236                   & 0.4136                  & 0.7687                         & 0.7155                         & 0.6712                         & 0.5549                  & 0.6463                   & 0.4383                  & 0.7659                  & 0.7252                   & 0.6708                  \\
                           & CT                        & \cellcolor{LightRed}0.7192                  & \cellcolor{LightRed}0.9021                   & \cellcolor{LightRed}0.6517                  & \cellcolor{LightRed}0.9060                          & \cellcolor{LightRed}0.9399                         & \cellcolor{LightRed}0.8754                         & 0.6664                  & \cellcolor{LightRed}0.8644                   & 0.5815                  & 0.8842                         & \cellcolor{LightRed}0.9153                         & 0.8396                         & 0.6662                  & \cellcolor{LightRed}0.8589                   & 0.5704                  & \cellcolor{LightRed}0.9095                  & \cellcolor{LightRed}0.9170                    & \cellcolor{LightRed}0.8740                   \\\hline\hline
\multirow{8}{*}\MovieTweetings             & \NEUMF                     & 0.4833                  & 0.8343                   & 0.3486                  & 0.7687                         & 0.8835                         & 0.6645                         & 0.5173                  & 0.8161                   & 0.3974                  & 0.8733                         & 0.8959                         & 0.8024                         & 0.5231                  & 0.8602                   & 0.3856                  & 0.8308                  & 0.9124                   & 0.7674                  \\
                           & \WIDE                      & 0.4297                  & 0.7824                   & 0.3078                  & 0.6883 & 0.8274 & 0.5702 & 0.4344                  & 0.7572                   & 0.3041                  & 0.6852 & 0.7908 & 0.5676 & 0.4234                  & 0.7276                   & 0.3032                  & 0.6883                  & 0.7809                   & 0.5577                  \\
                           & \DEEPFM                    & 0.4266                  & 0.781                    & 0.3074                  & 0.6781                         & 0.8211                         & 0.5545                         & 0.4391                  & 0.7556                   & 0.3153                  &0.6906 & 0.7896 & 0.5797 & 0.4125                  & 0.7253                   & 0.2994                  & 0.6828                  & 0.7737                   & 0.5505                  \\
                           & \AFN                       & 0.4094                  & 0.7672                   & 0.2947                  & 0.6937                         & 0.8117                         & 0.5664                         & 0.4453                  & 0.7522                   & 0.3132                  & 0.6938 & 0.7908 & 0.5658 & 0.4156                  & 0.7307                   & 0.3018                  & 0.6789                  & 0.7795                   & 0.5339                  \\
                           & \TANP                      & 0.4727                  & 0.8567                   & 0.3386                  & 0.7727                         & 0.9037                         & 0.6856                         & 0.552                   & 0.8281                   & 0.4566                  & 0.758                          & 0.8774                         & 0.6347                         & 0.5174                  & 0.8625                   & 0.398                   & 0.7217                  & 0.8964                   & 0.6318                  \\
                           & \MELU                      & 0.4829                  & 0.5275                   & 0.362                   & 0.761                          & 0.6679                         & 0.6639                         & 0.5073                  & 0.5657                   & 0.3998                  & 0.7585                         & 0.6901                         & 0.6774                         & 0.5122                  & 0.5391                   & 0.3769                  & 0.7488                  & 0.6604                   & 0.644                   \\
                           & \MAMO                      & 0.4789                  & 0.5265                   & 0.3468                  & 0.7567 & 0.6476 & 0.6404 & 0.482                   & 0.5275                   & 0.3564                  & 0.7555                         & 0.6513                         & 0.6394                         & 0.4633                  & 0.5233                   & 0.3351                  & 0.7576                  & 0.6481                   & 0.6421                  \\
                           & \CT                        & 0.5625                  & 0.8818                   & 0.4707                  & 0.7917                         & 0.9152                         & 0.7163                         & 0.6145                  & 0.875                    & 0.5                     & 0.8783                         & 0.9211                         & 0.8368                         & 0.58                    & 0.8863                   & 0.4759                  & 0.85                    & 0.9302                   & 0.7893                  \\\hline\hline
\multirow{8}{*}\Bookcrossing               & \NEUMF                     & 0.4867                  & 0.8493                   & 0.3643                  & 0.7125                         & 0.8872                         & 0.5868                         & 0.4571                  & 0.852                    & 0.3308                  & 0.6986                         & 0.8873                         & 0.5693                         & 0.4645                  & 0.8637                   & 0.3379                  & 0.6459                  & 0.8864                   & 0.4789                  \\
                           & \WIDE                      & 0.4761                  & 0.8461                   & 0.3567                  & 0.7092                         & 0.8864                         & 0.584                          & 0.4465                  & 0.8507                   & 0.3204                  & 0.6923                         & 0.8859                         & 0.5634                         & 0.4695                  & 0.8635                   & 0.3429                  & 0.651                   & 0.8867                   & 0.4813                  \\
                           & \DEEPFM                    & 0.4788                  & 0.848                    & 0.3594                  & 0.7103                         & 0.888                          & 0.5855                         & 0.4741                  & 0.8423                   & 0.3562                  & 0.7106                         & 0.8831                         & 0.5834                         & 0.4641                  & 0.8648                   & 0.331                   & 0.6496                  & 0.8871                   & 0.4825                  \\
                           & \AFN                       & 0.4758                  & 0.8455                   & 0.3518                  & 0.7081                         & 0.8849                         & 0.5795                         & 0.4477                  & 0.8527                   & 0.3208                  & 0.6926                         & 0.8881                         & 0.5624                         & 0.4749                  & 0.865                    & 0.342                   & 0.6543                  & 0.887                    & 0.4835                  \\
                           & \TANP                      & 0.4944                  & 0.8582                   & 0.3791                  & 0.7413                         & 0.8994                         & 0.63                           & 0.4957                  & 0.8755                   & 0.3793                  & 0.736                          & 0.9029                         & 0.6229                         & 0.644                   & 0.9245                   & 0.5303                  & 0.7548                  & 0.9198                   & 0.6423                  \\
                           & \MELU                      & 0.4056                  & 0.4836                   & 0.2936                  & 0.6611                         & 0.5891                         & 0.5262                         & 0.4875                  & 0.5235                   & 0.3481                  & 0.6875                         & 0.6157                         & 0.5473                         & 0.4432                  & 0.4922                   & 0.3299                  & 0.7095                  & 0.6148                   & 0.5825                  \\
                           & \MAMO                      & 0.4946                  & 0.3253                   & 0.4022                  & 0.8357                         & 0.4633                         & 0.7945                         & 0.5176                  & 0.3429                   & 0.4319                  & 0.8408                         & 0.4783                         & 0.8014                         & 0.5004                  & 0.3261                   & 0.4154                  & 0.8358                  & 0.4592                   & 0.7956                  \\
                           & \CT                        & 0.5284                  & 0.8662                   & 0.4289                  & 0.7472                         & 0.9016                         & 0.6453                         & 0.5679                  & 0.8911                   & 0.4747                  & 0.7597                         & 0.9137                         & 0.6712                         & 0.6797                  & 0.9435                   & 0.586                   & 0.7951                  & 0.9404                   & 0.7029    \\\hline             
\end{tabular}
}
\end{table*}
}



%Moreover, we are not sure whether complex heterogeneous interactions exist in them. 

%Most recommender systems \cite{NCF, WIDE, deepFM} only consider single type of interaction between users and items. While some other systems \cite{neighbor, metahin} construct complex structure to represent heterogeneous interactions in recommendation scenario. 
%However, lots of heterogeneous interactions are not observable in cold-start problem, it may fail to construct a reliable HIN.
%Moreover, it is possible that some interactions have noises and not conducive to prediction. For example, in a family, a mother has preference to buy a Robot Vacuum to do housework and this mother-son interaction has little impact on the son who has deep interests in games.
%The challenge lies in how to utilize existing limited interactions to identify useful heterogeneous interactions and weight them by their importance. 

%We propose to let model itself learn useful interactions and identify which interactions contribute most to estimate users' preference.
%Our work is inspired by the non-parametric transformers \cite{NPT}, which learns from entire dataset and utilize attention between datapoints to make prediction. 
%However, transformer is often designed for sequence data which is order dependent. Rating prediction for a set of users and items requires model to be order independent. The model has to give the invariant ratings when input order are changed. 
%Set transformer \cite{settransformer} is specially designed to model interactions among elements with property of permutation invariant. This is in line with the characteristics of the recommendation tasks. Thus we devise cube transformers which can model heterogeneous interactions via different attention layers to solve challenge. The proposed model follows permutation invariance and can provide shuffled input with consistent rating prediction.

%side information
%To solve the cold-start problem, content-based systems \cite{contentbase1, contentbase2, contentbase3} are leveraging side information into the model. They take use of user profile information (e.g., age, gender) or item content information (e.g., publication year, genre) to make recommendation. For one thing, side information cannot be obtained all the time since we often do not have access to user profile information for protection of personal privacy. For another thing, the model is hard to capture users' preference due to only using side information, which may lead to make similar recommendations for users with variant preferences. Consider two female users of an online shop who are both twenty years old students. One women purchased a few clothes and the other purchased some delicious food. However, due to limit products they have bought, there is a high probability that the system may recommend books to them considering their age and occupation. 


%In a movie recommendation website, users' preference for movies may depend on item features (e.g., actor,director of movies), intuitively. It indicates interactions between users and item features may contribute to predict ratings.
 %The challegnge is further exacerbated since few interactions can be observed in cold-start scenario.
 %但是这样的社区结构在冷启动的场景下不易获得，且不清楚是否存在社区结构。所以在特定场景下，找出有什么样的关系会影响到推荐是很有挑战性的。(并且在冷启动场景下，通常这样的关系很稀少，这加剧了挑战。)
%e.g., NCF \cite{NCF}, Wide\&Deep \cite{WIDE} and DeepFM \cite{deepFM}. 
%cite melu intro first paragraph
%cf

%\ding{172} We propose a novel framework, Cube Transformer (\CT) with Mask. We leverage stochastic target rating masks to indicate which ratings \CT is expected to predict. %cold start recommendation?meta-model?
%\ding{173} We design three multi-head self-attention layers to learn the attention between users, items and features, respectively, which can make use of interactions between instances (i.e., users, items and features) to improve the rating prediction.
%\ding{174}  %zero shot experiments, test without any prior knowledge
%1.(框架)设计了一个新框架解决推荐系统中的冷启动问题， 以解决xxxx三种冷启动的情况。我们设计了一个采样器，用来为new arrival user/item 产生预测的context，形成一个推荐任务，和一个多任务的元模型，可统一的为三种冷启动做出推荐。 并提出了相应的训练算法。
%2.（模型）设计了一个基于transformer的元模型，包含三种attention layer， 通过分别评估user item feature三个维度的相似性来对冷启动任务做出推荐。并证明了在一个推荐任务中，预测结果对context 的不变性/等变性。
%3.实验

\subsection{Transformer} %Transformer for Recommendation
\label{subsec:transformer}
%TODO
In our work, we propose Cube Transformer to model heterogeneous interactions.  Transformer \cite{attention} based solely on attention mechanisms, is a powerful tool for language model. 
%DELETE
Recently, it has been widely used in broad fields, e.g. tabular data. 
%In \CT, we get a tabular data after feature processing. 
A comprehensive survey of transformer  for tabular data representations can be found in \cite{survey}. 
Non-parametric transformers (NPTs) \cite{NPT} learn from data how to make use of other datapoints for prediction. They use multi-head self-attention to model interactions between datapoints and a stochastic masking mechanism is used to train objective for NPTs. 
Set Transformer \cite{settransformer} is designed to model interactions among elements in the permutation invariant input set. It is a significant property for recommending a set of users or items.
%多加一点
Transformer is used in recommendation system in recent years. NI-CTR~\cite{neighbor} predicts rating via graph-masked transformer. The transformer are able to learn neighbor representations to enhance feature interaction. BERT4Rec~\cite{BERT4REC} is a sequential recommendation model which can utilize deep bidirectional self-attention to model user behavior sequences.
However, transformer has not applied to tabular data for recommendation yet. Our work is the first to explore.



\begin{table*}[h]
\small
\centering
\caption{Performance in Three Cold-Start Scenarios on MovieLens}
\label{tab:result:movielens}
\begin{tabular}{c|c|c c c|c c c|c c c}
\hline
 {Scenario} & {Approach} &  Pre.@5 & NDCG@5 & MAP@5 &  Pre.@7 & NDCG@7 & MAP@7 & Pre.@10 & NDCG@10 & MAP@10  \\ \hline
 \multirow{8}{*}{\UC}                  & \NEUMF                    & 0.4864                  & 0.7856                   & 0.3589                  & 0.5899                            & 0.8077                   & 0.4535                  & 0.7171                  & 0.8371                   & 0.5938               \\
                                
    & \WIDE                     & 0.6079                  & 0.8585                   & 0.5144                  & 0.6735                            & 0.8670                    & 0.5795                  & 0.7713                  & 0.8849                   & 0.6915                \\
  & \DEEPFM                   & 0.6060                   & 0.8562                   & 0.5088                  & 0.6748                            & 0.8666                   & 0.5773                  & 0.7707                  & 0.8848                   & 0.6909             \\
  & \AFN                      & 0.5899                  & 0.8479                   & 0.4862                  & 0.6669                            & 0.8606                   & 0.5628                  & 0.7712                  & 0.8808                   & 0.6869               \\
     & \TANP                     & 0.6270                   & \underline{0.8717}                   & 0.5333                  & 0.6879                            & \underline{0.8812}                   & 0.5930                   & 0.7797                  & \underline{0.8987}                   & 0.6994               \\
      & \MELU                     & \underline{0.7104}                  & 0.7852                   & \underline{0.6275}                  & \underline{0.7755}                            & 0.8114                   & \underline{0.7047}                  & \underline{0.8868}                  & 0.8589                   & \underline{0.8469}               \\
     & \MAMO                     & 0.5428                  & 0.6327                   & 0.4241                  & 0.6161                            & 0.6554                   & 0.4951                  & 0.7661                  & 0.7187                   & 0.6678               \\
      & \CT                       & \cellcolor{LightYellow}0.7192                  & \cellcolor{LightYellow}0.9021                   & \cellcolor{LightYellow}0.6517                  & \cellcolor{LightYellow}0.7907                            & \cellcolor{LightYellow}0.9144                   & \cellcolor{LightYellow}0.7296                  & \cellcolor{LightYellow}0.9060                   & \cellcolor{LightYellow}0.9399                   & \cellcolor{LightYellow}0.8754               \\\hline
 \multirow{8}{*}{\IC}                  & \NEUMF                    & 0.5039                  & 0.6645                   & 0.3731                  & 0.6604                            & 0.7306                   & 0.5360                   & 0.7864                  & 0.7662                   & 0.6972                 \\
                                
   & \WIDE                     & 0.4776                  & 0.6314                   & 0.3605                  & 0.5869                            & 0.6625                   & 0.4605                  & 0.7357                  & 0.7105                   & 0.6313                  \\
    & \DEEPFM                   & 0.4626                  & 0.6166                   & 0.3391                  & 0.5833                            & 0.6521                   & 0.4492                  & 0.7343                  & 0.7020                    & 0.6263                \\
 & \AFN                      & 0.4496                  & 0.6003                   & 0.3288                  & 0.5695                            & 0.6360                    & 0.4348                  & 0.7268                  & 0.6888                   & 0.6140                  \\
     & \TANP                     & 0.5488                  & \underline{0.8072}                   & 0.4257                  & 0.6323                            & \underline{0.8236}                   & 0.5051                  & 0.7544                  & 0.8528                   & 0.6492          \\
      & \MELU                     & \cellcolor{LightYellow}0.7119                  & 0.7856                   & \cellcolor{LightYellow}0.6280                   & \cellcolor{LightYellow}0.7760                             & 0.8118                   & \cellcolor{LightYellow}0.7047                  & \cellcolor{LightYellow}0.8874                  & \underline{0.8589}                   & \cellcolor{LightYellow}0.8473              \\
    & \MAMO                     & 0.5371                  & 0.6236                   & 0.4136                  & 0.6175                            & 0.6496                   & 0.4959                  & 0.7687                  & 0.7155                   & 0.6712                 \\
 & \CT                       & \underline{0.6664}                  & \cellcolor{LightYellow}0.8644                   & \underline{0.5815}                  & \underline{0.7540}                             & \cellcolor{LightYellow}0.8824                   & \underline{0.6732}                  & \underline{0.8842}                  & \cellcolor{LightYellow}0.9153                   & \underline{0.8396}           \\\hline
   \multirow{8}{*}{\UIC}                 & \NEUMF                    & 0.5049                  & 0.6695                   & 0.3756                  & 0.6599                            & 0.7337                   & 0.5380                   & 0.7875                  & 0.7691                   & 0.7009              \\
    & \WIDE                     & 0.4864                  & 0.6405                   & 0.3657                  & 0.5922                            & 0.6719                   & 0.4645                  & 0.7338                  & 0.7157                   & 0.6309           \\
  & \DEEPFM                   & 0.4657                  & 0.6200                     & 0.3377                  & 0.5825                            & 0.6561                   & 0.4455                  & 0.7355                  & 0.7059                   & 0.6247          \\
   & \AFN                      & 0.4745                  & 0.6334                   & 0.3583                  & 0.5747                            & 0.6594                   & 0.4514                  & 0.7161                  & 0.6998                   & 0.6131         \\
    & \TANP                     & 0.5371                  & \underline{0.8069}                   & 0.4120                   & 0.6283                            & \underline{0.8241}                   & 0.4995                  & 0.7467                  & 0.8516                   & 0.6420              \\
  & \MELU                     & \cellcolor{LightYellow}0.7102                  & 0.7842                   & \cellcolor{LightYellow}0.6267                  & \cellcolor{LightYellow}0.7771                            & 0.8111                   & \cellcolor{LightYellow}0.7048                  & \underline{0.8883}                  & \underline{0.8585}                   & \underline{0.8479}               \\
       & \MAMO                     & 0.5549                  & 0.6463                   & 0.4383                  & 0.6213 & 0.6655                   & 0.5033                  & 0.7659                  & 0.7252                   & 0.6708              \\
     & \CT                       & \underline{0.6662}                  & \cellcolor{LightYellow}0.8589                   & \underline{0.5704}                  & \underline{0.7650}                             & \cellcolor{LightYellow}0.8791                   & \underline{0.6818}                  & \cellcolor{LightYellow}0.9095                  & \cellcolor{LightYellow}0.9170                    & \cellcolor{LightYellow}0.8740                     \\\hline
\end{tabular}
\end{table*}


\begin{table*}[h]
\small
\centering
\caption{Performance in Three Cold-Start Scenarios on MovieTweetings}
\label{tab:result:movietweetings}
\begin{tabular}{c|c|c c c|c c c|c c c}
\hline
 {Scenario} & {Approach} &  Pre.@5 & NDCG@5 & MAP@5 &  Pre.@7 & NDCG@7 & MAP@7 & Pre.@10 & NDCG@10 & MAP@10 \\ \hline
\multirow{8}{*}{\UC}                  & \NEUMF                    & 0.4732                  & 0.8257                   & 0.3486                  & 0.6042                            & 0.8537                   & 0.4711                  & 0.7687                  & 0.8835                   & 0.6645                  \\
&  \WIDE                  & 0.4297    & 0.7824    & 0.3078   & 0.5446    & 0.7998     & 0.4096  & 0.6883  & 0.8274   & 0.5702    \\
& \DEEPFM                     & 0.4266    & 0.7810    & 0.3074   & 0.5346    & 0.7966     & 0.4004  & 0.6781  & 0.8211   & 0.5545    \\
 & \AFN                     & 0.4094    & 0.7672    & 0.2947   & 0.5246    & 0.7802     & 0.3813  & 0.6937  & 0.8117   & 0.5664    \\
 & \TANP                     & 0.4727                  & \underline{0.8567}                   & 0.3386                  & \underline{0.6234}                            & \underline{0.8785}                   & \underline{0.4863}                  & \underline{0.7727}                  & \underline{0.9037}                   & \underline{0.6856}                  \\
 & \MELU                     & \underline{0.4829}                  & 0.5275                   & \underline{0.3620}                   & 0.6098                            & 0.5885                   & 0.4681                  & 0.7610                   & 0.6679                   & 0.6639                  \\
  & \MAMO                    &0.4789	&0.5265	&0.3468	 &0.5808	&0.5698	&0.4407	 &0.7567	&0.6476	&0.6404         \\
 & \CT                       & \cellcolor{LightYellow}0.5625                  & \cellcolor{LightYellow}0.8818                   & \cellcolor{LightYellow}0.4707                  & \cellcolor{LightYellow}0.6280                             & \cellcolor{LightYellow}0.8901                   & \cellcolor{LightYellow}0.5284                  & \cellcolor{LightYellow}0.7917                  & \cellcolor{LightYellow}0.9152                   & \cellcolor{LightYellow}0.7163                  \\\hline
\multirow{8}{*}{\IC}                  & \NEUMF                    & 0.5173                  & 0.8161                   & 0.3974                  & {0.6024}                            & {0.8422}                   & 0.5053                  & {0.6986}                  & \underline{0.8873}                   & {0.5693}    \\
&  \WIDE                 & 0.4344    & 0.7572    & 0.3041   & 0.5246    & 0.7664     & 0.3833  & 0.6852  & 0.7908   & 0.5676     \\
& \DEEPFM                      & 0.4391    & 0.7556    & 0.3153   & 0.5391    & 0.7645     & 0.3975  & 0.6906  & 0.7896   & 0.5797     \\
& \AFN                      & 0.4453    & 0.7522    & 0.3132   & 0.5223    & 0.7592     & 0.3780  & 0.6938  & 0.7908   & 0.5658     \\
& \TANP                     & \underline{0.5520}                   & \underline{0.8281}                   & \underline{0.4566}                  & \underline{0.6371}                            & \underline{0.8438}                   & \underline{0.5271}                  & 0.7580                   & 0.8774                   & 0.6347                  \\
& \MELU                     & 0.5073                  & 0.5657                   & 0.3998                  & 0.6272                            & 0.6265                   & 0.5138                  & \underline{0.7585}                  & 0.6901                   & \underline{0.6774}                  \\
& \MAMO                     &0.4820	&0.5275	&0.3564	&0.5908	&0.5752	&0.4511	&0.7555	&0.6513	&0.6394         \\
& \CT                       & \cellcolor{LightYellow}0.6145                  & \cellcolor{LightYellow}0.8750                    & \cellcolor{LightYellow}0.5000                     &\cellcolor{LightYellow} 0.6957                            &\cellcolor{LightYellow} 0.8878                   &\cellcolor{LightYellow} 0.6047                  & \cellcolor{LightYellow}0.8783                  &\cellcolor{LightYellow} 0.9211                   & \cellcolor{LightYellow}0.8368                  \\\hline
\multirow{8}{*}{\UIC}                 & \NEUMF                    & {0.4645}                  & 0.8602                   & 0.3856                  & {0.5407}                            & \underline{0.8732}                   & {0.4037}                  & {0.6426}                  & {0.8893}                   &{0.4769}                  \\
& \WIDE                  & 0.4234    & 0.7276    & 0.3032   & 0.5112    & 0.7395     & 0.3706  & 0.6883  & 0.7809   & 0.5577    \\
 & \DEEPFM                     & 0.4125    & 0.7253    & 0.2994   & 0.5067    & 0.7360     & 0.3752  & 0.6828  & 0.7737   & 0.5505     \\
& \AFN                      & 0.4156    & 0.7307    & 0.3018   & 0.5179    & 0.7456     & 0.3777  & 0.6789  & 0.7795   & 0.5339     \\
& \TANP                     & \underline{0.5174}                  & \underline{0.8625}                   & \underline{0.3980}                   & 0.5311                            & 0.8669                   & 0.4061                  & 0.7217                  & \underline{0.8964}                   & 0.6318                  \\
& \MELU                     & 0.5122                  & 0.5391                   & 0.3769                  & \underline{0.5993}                            & 0.5949                   & \underline{0.4694}                  & 0.7488                  & 0.6604                   & \underline{0.6440}                   \\
& \MAMO                     & 0.4633                  & 0.5233                   & 0.3351                  & 0.5684                            & 0.5687                   & 0.4264                  & \underline{0.7576}                  & 0.6481                   & 0.6421                  \\
& \CT                       & \cellcolor{LightYellow}0.5800                    & \cellcolor{LightYellow}0.8863                   & \cellcolor{LightYellow}0.4759                  & \cellcolor{LightYellow}0.6829                            & \cellcolor{LightYellow}0.9008                   & \cellcolor{LightYellow}0.5817                  & \cellcolor{LightYellow}0.8500                    & \cellcolor{LightYellow}0.9302                   & \cellcolor{LightYellow}0.7893                  \\\hline
\end{tabular}
\end{table*}


\begin{table*}[h]
\small
\centering
\caption{Performance on Three Cold-Start Scenarios on Bookcrossing}
\label{tab:result:bookcrossing}
\begin{tabular}{c|c|c c c|c c c|c c c}
\hline
 {Scenario} & {Approach} &  Pre.@5 & NDCG@5 & MAP@5 &  Pre.@7 & NDCG@7 & MAP@7 & Pre.@10 & NDCG@10 & MAP@10 \\ \hline
 \multirow{8}{*}{\UC}                  & \NEUMF                    & 0.4867                  & 0.8493                   & 0.3643                  & 0.5755                            & 0.8641                   & 0.4403                  & 0.7125                  & 0.8872                   & 0.5868                  \\
& \WIDE                   & 0.4761    & 0.8461    & 0.3567   & 0.5673    & 0.8629     & 0.4339  & 0.7092  & 0.8864   & 0.5840   \\
&  \DEEPFM                    & 0.4788    & 0.8480    & 0.3594   & 0.5700    & 0.8639     & 0.4342  & 0.7103  & 0.8880   & 0.5855     \\
& \AFN                     & 0.4758    & 0.8455    & 0.3518   & 0.5626    & 0.8600     & 0.4211  & 0.7081  & 0.8849   & 0.5795     \\
& \TANP                     & {0.4944}                  & \underline{0.8582}                   & 0.3791                  & \underline{0.6107}                            & \underline{0.8771}                   & \underline{0.4786}                  & \underline{0.7413}                  & \underline{0.8994}                   & 0.6300                    \\
  & \MELU       &0.4472	&0.5238	&0.3542	  &0.5635	&0.5646	&0.4375	 &0.7139	&0.6250	&0.6172
           \\
 & \MAMO                     & \underline{0.4946}	&0.3253
	&\underline{0.4022}	&0.5398	&0.3830	&0.4336	&0.7106	&0.4633	&\underline{0.6364}                                 \\
 & \CT                       & \cellcolor{LightYellow}0.5284                  & \cellcolor{LightYellow}0.8662                   & \cellcolor{LightYellow}0.4289                  & \cellcolor{LightYellow}{0.6166}                            & \cellcolor{LightYellow}0.8799                   & \cellcolor{LightYellow}{0.5006}                  & \cellcolor{LightYellow}{0.7472}                  & \cellcolor{LightYellow}0.9016                   & \cellcolor{LightYellow}{0.6453}                  \\\hline
\multirow{8}{*}{\IC}                  & \NEUMF                    & 0.4571                  & 0.8520                    & 0.3308                  & 0.5514                            & 0.8651                   & 0.4072                  & 0.6986                  & 0.8873                   & 0.5693                  \\
& \WIDE                  & 0.4465    & 0.8507    & 0.3204   & 0.5482    & 0.8652     & 0.4069  & 0.6923  & 0.8859   & 0.5634  \\
& \DEEPFM                      & 0.4741    & 0.8423    & 0.3562   & 0.5627    & 0.8580     & 0.4251  & 0.7106  & 0.8831   & 0.5834  \\
& \AFN                      & 0.4477    & 0.8527    & 0.3208   & 0.5487    & 0.8666     & 0.4057  & 0.6926  & 0.8881   & 0.5624  \\
& \TANP                     & {0.4957}                  & \underline{0.8755}                   & {0.3793}                  & \underline{0.5941}                            & \underline{0.8877}                   & \underline{0.4673}                  & \underline{0.7360}                   & \underline{0.9029}                   & 0.6229                  \\
& \MELU &0.4812	&0.5456	&0.3541	 &0.5379	&0.5730	&0.3962	 &0.7000	&0.6267	&0.5919       
     \\
& \MAMO                     & \underline{0.5176}	&0.3429	&\underline{0.4319}	&0.5466	&0.3967	&0.4522	&0.7160	&0.4783	&\underline{0.6444}                  \\
& \CT                       & \cellcolor{LightYellow}0.5679                  & \cellcolor{LightYellow}0.8911                   & \cellcolor{LightYellow}0.4747                  & \cellcolor{LightYellow}0.6454                            & \cellcolor{LightYellow}0.8981                   & \cellcolor{LightYellow}0.5504                  & \cellcolor{LightYellow}0.7597                  & \cellcolor{LightYellow}0.9137                   & \cellcolor{LightYellow}0.6712                  \\\hline
 \multirow{8}{*}{\UIC}                 & \NEUMF                    & 0.4645                  & 0.8637                   & 0.3379                  & 0.5407                            & 0.8701                   & 0.3990                   & 0.6459                  & 0.8864                   & 0.4789                  \\
& \WIDE                   & 0.4695    & 0.8635    & 0.3429   & 0.5633    & 0.8739     & 0.4135  & 0.6510  & 0.8867   & 0.4813  \\
 &  \DEEPFM                    & 0.4641    & 0.8648    & 0.3310   & 0.5515    & 0.8735     & 0.4026  & 0.6496  & 0.8871   & 0.4825   \\
 & \AFN                      & 0.4749    & 0.8650    & 0.3420   & 0.5594    & 0.8732     & 0.4081  & 0.6543  & 0.8870   & 0.4835   \\
 & \TANP                     & \underline{0.6440}                   & \underline{0.9245}                   & \underline{0.5303}                  & \cellcolor{LightYellow}0.7029                            & \underline{0.9160}                    & \underline{0.6019}                  & \underline{0.7548}                  & \underline{0.9198}                   & 0.6423                  \\
& \MELU  &0.4784	&0.5165	&0.3620	 &0.5927	&0.5689	&0.4581	 &0.7378	&0.6346	&0.6355                         \\
& \MAMO                     & 0.5004	&0.3261	&0.4154	&0.6578	&0.3784	&0.4443	&0.7193	&0.4592	&\underline{0.6486}                  \\
 & \CT                       & \cellcolor{LightYellow}0.6797                  & \cellcolor{LightYellow}0.9435                   & \cellcolor{LightYellow}0.5860                   & \underline{0.7002}                            & \cellcolor{LightYellow}0.9431                   & \cellcolor{LightYellow}0.6118                  & \cellcolor{LightYellow}0.7951                  & \cellcolor{LightYellow}0.9404                   & \cellcolor{LightYellow}0.7029        \\\hline 
\end{tabular}
\end{table*}



%methodology

\section{Methodology}
\label{sec:method}
In this section, we present framework of heterogeneous interaction rating network to make cold-start rating prediction. We first give an overview and then describe detailed components for \HIRE. In the following, we show the learning algorithms to train model and apply the model to make cold-start rating prediction. Finally permutation equivariant of \HIM and time complexity are analyzed.

\subsection{Overview}
 

\subsection{Feature Processing.}
\label{generate}
We first construct a subset of user set $U$ and item set $I$. 
We devise a sampling strategy to generate user set $\mathcal{U}$ and item set $\mathcal{I}$ for one batch. 
%\rrcomment{What is the one-hop sampling strategy? one-hot encoding? Here, 'task' or 'batch'? }
On the one hand, we try to maximize interactions between the sampling users and items in a batch. Since more existing interactions have a higher probability of possessing more implicit interactions.
On the other hand, considering computational cost and limited observed interactions, we do not explore a more complicated sampling strategy.
A batch of $n$ users and $d$ items are generated with the following steps:
Let $n$ and $d$ denote the users and items size in generated set. $\mathcal{U}$ and $\mathcal{I}$ denote users and items set we have already sampled, respectively. Given observed interaction matrix $Y$ in large dataset, for a user $u$, there exists interactions with items in interaction matrix $Y$. 
We retrieve $d$ items from those have interactions with $u$ and constitutes item set $\mathcal{I}$. 
For each $i$ in set $\mathcal{I}$, we randomly retrieve $n-1$ users satisfying the number of interactions with set $\mathcal{I}$ is no less than a threshold.
 
The process to generate user and item set is depicted in Fig.~\ref{fig:matrix}. There is an example to illustrate the above process. The left figure refers to entire large dataset, while the right one is a generated set.
\begin{example}
Suppose we aim to sample a batch with $n=4$ users and $d=4$ items.
$u_1$ is first user randomly sampled from large dataset. A set of items $\{i_1,i_2,i_4,i_6\}$ having interactions with $u_1$ are retrieved to compose item set. 
For other users $u_2$ to $u_6$, they have 1, 1, 2, 2, 0 interactions with items in $\mathcal{I}$, respectively. We set threshold $\beta=1$, and randomly retrieve $\{u_3,u_4,u_5\}$ to constitute user set $\mathcal{U}$. The generated set is shown in Fig.~\ref{fig:matrix} (Right). 
%We sort remaining users by number of interactions they have with items in $\mathcal{I}$, and get $\{u_4, u_5, u_2, u_3, u_6\}$ have $\{2,2,1,1,1\}$ interactions in descending order. To get $3$ users, we randomly sample from the sorting list, and finally select $\{u_3,u_4,u_5\}$. Fig.~\ref{fig:matrix} (Right) shows a newly generated graph.
%Then for each $v$ in the set, select some users who have as much as possible interactions with these items. The unknown weight in the graph is the masked rating in matrix to predict. Then a masked rating matrix is constructed.
\end{example}

%We introduce a bipartite graph to represent these interactions between users and items as depicted in Fig.~\ref{fig:matrix} (Left). 





After generating user and item set, we construct $\mathcal{T}=\{\mathcal{U},\mathcal{I},\mathcal{R},\mathcal{E}\}$ with their features $\mathcal{E}$ and get $n\times d$ user-item pair. 
Their ratings $\mathcal{R}$ are divided into observed ratings $\mathcal{S}$ and masked ratings $\mathcal{Q}$.
Note if an user has no interaction with one item, we set a masked rating to this pair. 

User features contain different categories and each category are one-hot encoding.
User linear transformation $f_U^s: {e_u^s} \rightarrow x_u^s$ maps one-hot encoding to $f$-dimensional dense embedding, where $s$ refers to category of user feature.
Given a user $u$ who has $h_u$ category of features, the embedding for the user is defined as:
\vspace{-1.5ex}
\begin{align}
\vspace{-1.5ex}
    x_u&=[f_U^1(e_u^1),f_U^2(e_u^2),\dots,f_U^{h_u}(e_u^{h_u})].
\end{align}
Similarly, item linear transformation $f_I^t: {e_v^t} \rightarrow x_i^t$ is utilized to map one-hot encoding to $f$-dimensional dense embedding. For an item $i$ with $h_i$ contents, the embedding for the item is defined as:
\vspace{-1.5ex}
\begin{align}
\vspace{-1.5ex}
    x_i&=[f_I^1(e_i^1),f_I^2(e_i^2),\dots,f_I^{h_i}(e_i^{h_i})].
\end{align}
It has to be noticed that the original embedding $e_u^s$ and $e_i^t$ are all one-hot encoding and they can have different dimensions, while $x_u^s$ and $x_i^t$ all have the same size, namely, $f$.
We input one-hot rating or masked rating (zero vector) into rating linear transformation $f_{R}: r_{ui} \rightarrow x_{ui}$,
\begin{align}
    x_{ui}=f_{R}(r_{ui}),
\end{align}
where $x_{ui}\in \mathbb{R}^f$.
Embedding $h_{ui}$ for a pair of user $u$ and item $i$ is concatenated by their user embedding, item embedding and rating embedding as shown,
\vspace{-1.5ex}
\begin{align}
\vspace{-1.5ex}
   {h}_{ui}&=[x_u,x_i,x_{ui}].\label{eq:concate}
\end{align}
Suppose $h=h_u+h_i+h_r$, where $h_u$ and $h_i$ denotes the number categories of features for user and item, respectively. And $h_r=1$ denotes that rating has one category, generally. Let $e$ denotes one pair embedding dimension, we can easily have $e=h \times f$.
Then for all the user-item pairs, we can get embedding matrix $\mathcal{H}^{(0)} \in \mathbb{R}^{n \times d \times e}$ as input in heterogeneous interaction module.


\subsection{Training and Test}
\stitle{Model Training.}
In the training stage, given training batches $\mathcal{D}=\{\mathcal{T}_j\}_{j=1}^T$, and the number of epochs $L$, \HIRE is trained by optimizing MSELoss as follows:
\vspace{-1.5ex}
\begin{align}
\vspace{-1.5ex}
    \loss= \sum_{\mathcal{D}}\sum_{r_{ui} \in \mathcal{Q}} (r_{ui}-\hat{r}_{ui})^2, \label{loss}
\end{align}
where $\mathcal{Q}$ is masked rating set and $\mathcal{D}$ refers to training batches.
Algorithm 1 presents the training process.
In each epoch (line~\ref{line:train:start}-\ref{line:train:end}), there are $T$ batches. 
For each batch (line~\ref{line:train:task:start}-\ref{line:train:task:end}), we first construct input embedding matrix $\mathcal{H}(i)$ by generating embeddings via linear transformation in line~\ref{line:train:encoder}. Second, let $\mathcal{H}(i)$ go through $K$ \HIM blocks in line~\ref{line:train:cube:start}-\ref{line:train:cube:end}. Third, we map $\mathcal{H}(i)$ to one-dimensional rating $\hat{R}(i)$ in line~\ref{line:train:decoder}. In line~\ref{line:train:loss}-\ref{line:train:update}, we compute MSELoss for each $\hat{R}(i)$, accumulate them and get loss $\mathcal{L}$ to update model parameters.

\stitle{Model Test.}
In test stage, when new batch $\mathcal{T}^*$ comes, we can construct an embedding matrix $\mathcal{H}^*$. Ratings to be predicted are masked. 
It is worth to mention that the size of matrix can be decided by the number of new users and items and can be flexible. 
$\mathcal{H}^*$ input into $K$ \HIM blocks and following a MLP to get predicted rating. 

==> bak1.tex <==
\multirow{7}{*}{User cold-start}          & NeuMF      & $0.3328_{\small(.0106)}$ & $0.3887_{\small(.011)}$  & $0.2657_{\small(.0167)}$ & $0.4176_{\small(.0112)}$ & $0.3962_{\small(.0132)}$ & $0.3388_{\small(.0203)}$ & $0.5165_{\small(.0155)}$ & $0.4178_{\small(.0127)}$ & $0.4214_{\small(.0271)}$ \\
 & Wide\&Deep & $0.2852_{\small(.0161)}$ & $0.5408_{\small(.0197)}$ & $0.2161_{\small(.0008)}$ & $0.3759_{\small(.0231)}$ & $0.5528_{\small(.0273)}$ & $0.2517_{\small(.0196)}$ & $0.4746_{\small(.0678)}$ & $0.5666_{\small(.0416)}$ & $0.3258_{\small(.0504)}$ \\
 & DeepFM     & $0.2956_{\small(.0013)}$ & $0.5154_{\small(.0066)}$ & $0.187_{\small(.0079)}$  & $0.3511_{\small(.0125)}$ & $0.523_{\small(.0151)}$  & $0.212_{\small(.007)}$   & $0.4321_{\small(.0278)}$ & $0.5224_{\small(.0015)}$ & $0.2787_{\small(.0233)}$ \\
 & AFN        & $0.2205_{\small(.0714)}$ & $0.497_{\small(.0354)}$  & $0.1462_{\small(.0644)}$ & $0.3195_{\small(.0414)}$ & $0.5063_{\small(.0264)}$ & $0.1856_{\small(.0452)}$ & $0.421_{\small(.0066)}$  & $0.5238_{\small(.008)}$  & $0.2573_{\small(.0277)}$ \\
 & MAMO       & $0.4177_{\small(.0189)}$ & $0.2995_{\small(.0254)}$ & $0.3232_{\small(.0195)}$ & $0.5573_{\small(.0191)}$ & $0.3494_{\small(.0285)}$ & $0.4562_{\small(.0185)}$ & $0.7209_{\small(.0151)}$ & $0.4118_{\small(.0274)}$ & $0.6529_{\small(.0154)}$ \\
 & TaNP       & $0.4118_{\small(.003)}$  & $0.8504_{\small(.0145)}$ & $0.3338_{\small(.0039)}$ & $0.4598_{\small(.0054)}$ & $0.8601_{\small(.011)}$  & $0.3626_{\small(.0131)}$ & $0.5288_{\small(.021)}$  & $0.8712_{\small(.0072)}$ & $0.416_{\small(.0329)}$  \\
 & MeLU       & $0.4651_{\small(.0416)}$ & $0.586_{\small(.0709)}$  & $0.3534_{\small(.044)}$  & $0.5282_{\small(.0779)}$ & $0.6079_{\small(.0737)}$ & $0.4079_{\small(.0662)}$ & $0.6295_{\small(.114)}$  & $0.6466_{\small(.0798)}$ & $0.5096_{\small(.1286)}$ \\
 & HIRE       & $0.5447_{\small(.0476)}$ & $0.8799_{\small(.0248)}$ & $0.4715_{\small(.0667)}$ & $0.6177_{\small(.0324)}$ & $0.8939_{\small(.023)}$  & $0.5304_{\small(.0538)}$ & $0.7075_{\small(.0409)}$ & $0.9208_{\small(.0196)}$ & $0.6303_{\small(.0369)}$




  \\ \midrule %\hline\hline
\multirow{7}{*}{Item cold-start}          & NeuMF      & $0.407_{\small(.0066)}$  & $0.416_{\small(.1321)}$  & $0.3282_{\small(.0414)}$ & $0.5142_{\small(.0225)}$ & $0.4362_{\small(.1374)}$ & $0.4303_{\small(.0773)}$ & $0.593_{\small(.0868)}$  & $0.462_{\small(.1324)}$  & $0.5104_{\small(.1282)}$ \\
 & Wide\&Deep & $0.5007_{\small(.0786)}$ & $0.8014_{\small(.0095)}$ & $0.406_{\small(.1092)}$  & $0.5691_{\small(.1031)}$ & $0.8059_{\small(.0096)}$ & $0.462_{\small(.144)}$   & $0.6166_{\small(.1141)}$ & $0.8047_{\small(.0058)}$ & $0.5128_{\small(.1549)}$ \\
 & DeepFM     & $0.5246_{\small(.0813)}$ & $0.811_{\small(.0162)}$  & $0.4456_{\small(.1153)}$ & $0.5704_{\small(.1196)}$ & $0.8156_{\small(.0181)}$ & $0.4862_{\small(.1558)}$ & $0.6146_{\small(.1306)}$ & $0.8123_{\small(.0219)}$ & $0.5246_{\small(.1678)}$ \\
 & AFN        & $0.4915_{\small(.071)}$  & $0.8018_{\small(.0178)}$ & $0.404_{\small(.0908)}$  & $0.5395_{\small(.0998)}$ & $0.8083_{\small(.0187)}$ & $0.4395_{\small(.1303)}$ & $0.6201_{\small(.1103)}$ & $0.8129_{\small(.0187)}$ & $0.5141_{\small(.1522)}$ \\
 & MAMO       & $0.4129_{\small(.0062)}$ & $0.281_{\small(.0049)}$  & $0.3246_{\small(.0051)}$ & $0.5462_{\small(.0041)}$ & $0.324_{\small(.0036)}$  & $0.4498_{\small(.0071)}$ & $0.716_{\small(.0036)}$  & $0.3942_{\small(.0086)}$ & $0.6418_{\small(.0019)}$ \\
 & TaNP       & $0.4116_{\small(.0315)}$ & $0.8545_{\small(.0132)}$ & $0.3125_{\small(.0152)}$ & $0.4506_{\small(.0174)}$ & $0.8618_{\small(.0129)}$ & $0.3287_{\small(.029)}$  & $0.5194_{\small(.0435)}$ & $0.8713_{\small(.0122)}$ & $0.3848_{\small(.0504)}$ \\
 & MeLU       & $0.4925_{\small(.0577)}$ & $0.6159_{\small(.0289)}$ & $0.3764_{\small(.0517)}$ & $0.5204_{\small(.082)}$  & $0.6258_{\small(.0245)}$ & $0.3915_{\small(.0639)}$ & $0.6058_{\small(.126)}$  & $0.6565_{\small(.0362)}$ & $0.4769_{\small(.1326)}$ \\
 & HIRE       & $0.5837_{\small(.0338)}$ & $0.8925_{\small(.0056)}$ & $0.5174_{\small(.0327)}$ & $0.6418_{\small(.0244)}$ & $0.9057_{\small(.0057)}$ & $0.5649_{\small(.0206)}$ & $0.722_{\small(.0471)}$  & $0.9262_{\small(.0065)}$ & $0.6519_{\small(.0497)}$   \\\midrule %\hline\hline
\multirow{7}{*}{User \& item cold-start} & NeuMF      & $0.3829_{\small(.0097)}$ & $0.4617_{\small(.1013)}$ & $0.2976_{\small(.0105)}$ & $0.4342_{\small(.012)}$  & $0.4728_{\small(.1078)}$ & $0.3274_{\small(.0229)}$ & $0.4922_{\small(.0074)}$ & $0.4871_{\small(.1083)}$ & $0.3661_{\small(.017)}$  \\
 & Wide\&Deep & $0.4037_{\small(.0841)}$ & $0.6702_{\small(.1851)}$ & $0.3304_{\small(.0696)}$ & $0.4672_{\small(.1132)}$ & $0.6494_{\small(.1911)}$ & $0.3757_{\small(.1037)}$ & $0.5275_{\small(.1163)}$ & $0.6632_{\small(.1626)}$ & $0.4033_{\small(.1389)}$ \\
 & DeepFM     & $0.3927_{\small(.0771)}$ & $0.6848_{\small(.0731)}$ & $0.3018_{\small(.071)}$  & $0.475_{\small(.0294)}$  & $0.69_{\small(.0838)}$   & $0.3649_{\small(.0429)}$ & $0.5414_{\small(.0965)}$ & $0.6907_{\small(.1017)}$ & $0.5071_{\small(.2051)}$ \\
 & AFN        & $0.3476_{\small(.0396)}$ & $0.589_{\small(.1211)}$  & $0.2815_{\small(.0301)}$ & $0.3505_{\small(.0193)}$ & $0.5866_{\small(.1194)}$ & $0.2651_{\small(.0085)}$ & $0.3988_{\small(.0317)}$ & $0.6043_{\small(.1147)}$ & $0.2839_{\small(.0289)}$ \\
 & MAMO       & $0.41_{\small(.0087)}$   & $0.3256_{\small(.0632)}$ & $0.3026_{\small(.0376)}$ & $0.5167_{\small(.0763)}$ & $0.3699_{\small(.0534)}$ & $0.4101_{\small(.0934)}$ & $0.7178_{\small(.0154)}$ & $0.4485_{\small(.0724)}$ & $0.638_{\small(.0391)}$  \\
 & TaNP       & $0.5114_{\small(.0174)}$ & $0.8812_{\small(.065)}$  & $0.4365_{\small(.0083)}$ & $0.5153_{\small(.0214)}$ & $0.8774_{\small(.0447)}$ & $0.4286_{\small(.0456)}$ & $0.5484_{\small(.0676)}$ & $0.878_{\small(.025)}$   & $0.4531_{\small(.0856)}$ \\
 & MeLU       & $0.4335_{\small(.0436)}$ & $0.5465_{\small(.0146)}$ & $0.3349_{\small(.0293)}$ & $0.4992_{\small(.0928)}$ & $0.5716_{\small(.008)}$  & $0.3784_{\small(.0788)}$ & $0.5758_{\small(.1438)}$ & $0.5993_{\small(.0351)}$ & $0.4562_{\small(.1635)}$ \\
 & HIRE       & $0.6077_{\small(.0333)}$ & $0.906_{\small(.0025)}$  & $0.5529_{\small(.0322)}$ & $0.6903_{\small(.043)}$  & $0.9209_{\small(.0051)}$ & $0.6284_{\small(.0405)}$ & $0.7636_{\small(.0689)}$ & $0.9392_{\small(.0064)}$ & $0.7015_{\small(.0812)}$

